On the Structure of Optimal Transportation Plans between Discrete Measures

In this paper, we prove a structure theorem for discrete optimal transportation plans. We show that, given any pair of discrete probability measures and a cost function, there exists an optimal transportation plan that can be expressed as the sum of two deterministic plans. As an application, we estimate the infinity-Wasserstein distance between two discrete probability measures $\mu$ and $\nu$ with the $p$-Wasserstein distance, times a constant depending on $\mu$, $\nu$, and the fixed cost function.

==> scarti.tex <==
In what follows, we focus our attention on the euclidean cost function
\[
c(x,y)=|x-y|:=\sqrt{\sum^n_{i=1}(x_i-y_i)^2},
\]
and to its powers
\[
c_p(x,y)=|x-y|^p,
\]
hence let $X\subset \erre^n$.

\noindent In this framework, we prove the discrete version of the estimate presented for absolutely continuous measures in \cite{bouchitte07}. 

\noindent We recall that, given two measures $\mu$ and $\nu$, the $p-th$ power Wasserstein distance is defined as
\[
W_p^p(\mu,\nu):=\min_{\pi\in\Pi(\mu,\nu)}T_{c_p}(\pi)=\min_{\pi\in\Pi(\mu,\nu)}\sum_{(x,y)\in X\times X}|x-y|^p\pi_{x,y}
\]
Similarly
\[
W^{(\infty)}(\mu,\nu):=\min_{\pi\in\Pi(\mu,\nu)}T^{(\infty)}(\pi),
\]
where
\[
T^{(\infty)}(\pi):=\max\bigg\{|x-y|\, \Big| \,\,(x,y)\in spt(\pi)\bigg\}.
\]

